Collaborative Learning for 3D Hand-Object Reconstruction and Compositional Action Recognition from Egocentric RGB Videos Using Superquadrics

With the availability of egocentric 3D hand-object interaction datasets, there is increasing interest in developing unified models for hand-object pose estimation and action recognition. However, existing methods still struggle to recognise seen actions on unseen objects due to the limitations in representing object shape and movement using 3D bounding boxes. Additionally, the reliance on object templates at test time limits their generalisability to unseen objects. To address these challenges, we propose to leverage superquadrics as an alternative 3D object representation to bounding boxes and demonstrate their effectiveness on both template-free object reconstruction and action recognition tasks. Moreover, as we find that pure appearance-based methods can outperform the unified methods, the potential benefits from 3D geometric information remain unclear. Therefore, we study the compositionality of actions by considering a more challenging task where the training combinations of verbs and nouns do not overlap with the testing split. We extend H2O and FPHA datasets with compositional splits and design a novel collaborative learning framework that can explicitly reason about the geometric relations between hands and the manipulated object. Through extensive quantitative and qualitative evaluations, we demonstrate significant improvements over the state-of-the-arts in (compositional) action recognition.

==> tex/checklist.tex <==
\section{Reproducibility Checklist}

This paper:

\begin{itemize}
\item includes a conceptual outline and/or pseudocode description of AI methods introduced. [\textbf{yes}]
\item clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. [\textbf{yes}]
\item provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. [\textbf{yes}]
\end{itemize}

\noindent
Does this paper make theoretical contributions? [\textbf{no}]	

\noindent
Does this paper rely on one or more datasets? [\textbf{yes}]
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets. [\textbf{yes}]
\item All novel datasets introduced in this paper are included in a data appendix. [\textbf{NA}]
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [\textbf{NA}]
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. [\textbf{yes}]
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available.[\textbf{yes}]
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. [\textbf{NA}]
\end{itemize}

\noindent
Does this paper include computational experiments? [\textbf{yes}]

\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. [\textbf{yes}]
\item All source code required for conducting and analyzing the experiments is included in a code appendix. [\textbf{yes}]
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [\textbf{no}]
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. [\textbf{yes}]
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. [\textbf{yes}]
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. [\textbf{yes}]
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. [\textbf{yes}]
\item This paper states the number of algorithm runs used to compute each reported result. [\textbf{yes}]
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information.  [\textbf{yes}] 
%Following previous works \cite{sun2019deep, liu2021deep}, we adopt the widely used average precision (AP) as the metric. Additionally, we present computational cost analysis (\#Params. and GFLOPs) in Table 4 in the main text. 
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). [\textbf{no}] 
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. [\textbf{yes}]
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. [\textbf{partial}]
\end{itemize}
